Decorrelation with conditional normalizing flows

The sensitivity of many physics analyses can be enhanced by constructing discriminants that preferentially select signal events. Such discriminants become much more useful if they are uncorrelated with a set of protected attributes. In this paper we show that a normalizing flow conditioned on the protected attributes can be used to find a decorrelated representation for any discriminant. As a normalizing flow is invertible the separation power of the resulting discriminant will be unchanged at any fixed value of the protected attributes. We demonstrate the efficacy of our approach by building supervised jet taggers that produce almost no sculpting in the mass distribution of the background.

==> appendicies/dataset.tex <==
\section{Dataset details}
\label{app:dataset}
Both signal and background were generated by \textsc{Pythia} at $s=\sqrt{13}$ TeV with a detector simulated by \textsc{Delphes}. Jets are reconstructed using \textsc{FastJet}~\cite{cacciari2012fastjet,cacciari2006dispelling} and clustered using the anti-\textit{kt} algorithm~\cite{cacciari2008anti} with $R = 1.0$. Each jet is required to have transverse momentum $p_T \in [300, 400]$ GeV and mass  $m \in [50,300]$. For each jet ten substructure variables are calculated and used as input to the machine learning classifiers, these variables are the same as those used in previous studies of decorrelation~\cite{ATL-PHYS-PUB-2018-014, mode, disco}. The invariant mass distribution is shown in Fig.~\ref{fig:mass_only}

\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth]{figures/mass_only.pdf}
    \caption{The invariant mass distribution for the background samples without applying any selection.}
    \label{fig:mass_only}
\end{figure}

==> appendicies/disco_levels.tex <==
\section{DisCo}
\label[]{app:disco_app}

Looking at different cuts on the classifier output for a different value of the DisCo loss. \sam{Describe more.}

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{figures/multi_cuts_disco_4.pdf}
    \caption{The mass distribution for different levels of rejection as defined by the thresholds of the quantile regression, which were set to the $50, 90, 95, 99$th quantiles. The mass distribution after applying cuts from a classifier trained with DisCo decorrelation ($\alpha=100$) and corrected with a conditional normalizing flow (cf-DisCo) and conditional quantile regression (qr-DisCo). Random bounds are defined by sampling the same number of statistics randomly $100$ times per threshold. 
    }
    \label{fig:multi_cuts} 
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{figures/quantile_quantified_disco_4.pdf}
    \caption{
        The performance of a DisCo trained classifier with $\alpha=100$ and both quantile regression and a flow decorrelated output at $50, 90, 95, 99\%$ background rejection. 
    }
    \label{fig:multi_cuts_200} 
\end{figure}

==> preamble.tex <==
\usepackage{lmodern}
\usepackage[T1]{fontenc}
\usepackage{amsmath}
\usepackage{amssymb}
%\usepackage[a4paper]{geometry}

\usepackage{url}
\usepackage{longtable}
\usepackage{multirow}
\usepackage{caption}
\usepackage[labelformat=simple]{subcaption}
\renewcommand\thesubfigure{(\alph{subfigure})}

\usepackage[nodayofweek]{datetime}
\usepackage{enumerate}
\usepackage{xspace}
\usepackage{xcolor}
\usepackage{graphicx}
\usepackage[pdftex,hidelinks]{hyperref}
\usepackage{bookmark}

\usepackage{float}
\usepackage[capitalise]{cleveref}

% \setlength{\mathindent}{8ex}

\newcommand{\angstrom}{\textup{\AA}}
\newcommand*\rfrac[2]{{}^{#1}\!/_{#2}}
\newcommand*\doublehat[1]{\ensuremath{\hat{\hat{#1}}}}

\newcommand\sam[1]{\textcolor{red}{#1}}
\newcommand\mass{$\boldsymbol{m}$}


\linespread{1.5}
\frenchspacing


\usepackage[backend=biber,giveninits=true,doi=false,sorting=none,style=numeric-comp]{biblatex}
\DeclareFieldFormat[article]{citetitle}{\textit{#1}\isdot}
\DeclareFieldFormat[article]{title}{\textit{#1}\isdot}
\DeclareFieldFormat[unpublished]{citetitle}{\textit{#1}\isdot}
\DeclareFieldFormat[unpublished]{title}{\textit{#1}\isdot}
\DeclareFieldFormat[inproceedings]{citetitle}{\textit{#1}\isdot}
\DeclareFieldFormat[inproceedings]{title}{\textit{#1}\isdot}

\DeclareNameAlias{author}{last-first}

\addbibresource{bib/rodem.bib}


==> tex/checklist.tex <==
\section*{Checklist}


% %%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
% %%% END INSTRUCTIONS %%%


\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{See conclusion section.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNo{We do not forsee any.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
        \item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{Code will be made publicly available with the camera ready version.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{Given the limited space in the main body this is given in App.~\ref{app:model_settings}.}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{Yes, ten random seeds were run for every experiment.}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerNo{Everything is public.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{The training utilities will be made public.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{All data was publicly available.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{Physics data.}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}
